A Prompt Response to the Demand for Automatic Gender-Neutral Translation

Gender-neutral translation (GNT) that avoids biased and undue binary assumptions is a pivotal challenge for the creation of more inclusive translation technologies. Advancements for this task in Machine Translation (MT), however, are hindered by the lack of dedicated parallel data, which are necessary to adapt MT systems to satisfy neutral constraints. For such a scenario, large language models offer hitherto unforeseen possibilities, as they come with the distinct advantage of being versatile in various (sub)tasks when provided with explicit instructions. In this paper, we explore this potential to automate GNT by comparing MT with the popular GPT-4 model. Through extensive manual analyses, our study empirically reveals the inherent limitations of current MT systems in generating GNTs and provides valuable insights into the potential and challenges associated with prompting for neutrality.

==> backup.tex/GNT-prompting-Andrea.tex <==
\section{\bs{GNT prompting}}
\label{sec:gnt-prompting}


\ap{For GNT, we tested three prompts with two sets of shots.\footnote{\ap{We use 3-shots prompts, which emerged as a valid compromise between performance and prompt length in our preliminary experiments. \textbf{Si potrebbe elaborare dicendo che gli esempi in questo caso sono manually crafted, quindi è costoso produrne in quantità maggiori, ma non so se abbiamo lo spazio per farlo/ci interessa. Può andare nelle limitations.}}} Examples of each prompt are available in Table \ref{tab:prompts-in-domain}.}


\ap{• \texttt{contr}: following \citet{sanchez_gender-specific_2023}, we ask the models to provide a contrastive pair of translations for each source sentence -- a gendered one, and a neutral one -- without providing any information about the task.} %The models are supposed to identify the pattern in the examples and to reproduce it.


\ap{• \texttt{CoT-1}: a Chain-of-Thought (CoT) prompt \citep{wei_chain--thought_2023} based on the GNT task description. The system is expected to identify English terms in the source sentence which could possibly be translated as marked in Italian and to elaborate gender-neutral translations before the generation of the final translation.}

\ap{• \texttt{CoT-2}: this CoT replicates how humans instinctively perform GNTs \citep{piergentili-etal-2023-gender,paolucci-etal-2023-gender}, i.e. by first producing a gendered translation and subsequently \textit{neutralizing} gendered terms to produce the final translation.}


\ap{As English emerged as the most effective language for prompting \citep{shi_language_2022,zhang_prompting_2023}, we use English instructions in our prompts, except for the Italian examples in the task demonstrations.} \ap{As for the examples, we developed two sets of shots that differ only for the English terms which require a GNT and their translations into Italian. One set includes terms which exist in GeNTE set (we report the number of occurrences in Table \ref{tab:occurrences}), while the other features terms which do not. This allows to investigate the impact of example choice on a complex task of text generation. }
%i.e. whether choosing examples too similar to the test data can lead to overfitting-like scenario.

==> backup.tex/abstract-matteo.tex <==
\mn{Despite the 
impressive and 
steady progress in recent years, 
translation technologies still grapple 
%machine translation (MT) systems still grapple 
with well-known issues inherent in their data-driven nature. The lack of parallel data for specific tasks or domains is indeed one of the main problems that limit their overall reliability or even their usability in narrow or highly constrained application contexts. These, however, are the scenarios in which large language models (LLMs) offer hitherto unforeseen possibilities. Although they still lag behind traditional supervised 
machine translation (MT) systems
%MT systems 
in general translation tasks, they come with the distinct advantage of being versatile in various (sub-)tasks when provided with explicit instructions and minimal examples. In this paper, we explore this potential by comparing 
%three
\bs{two}
state-of-the-art encoder-decoder MT systems 
%(Google Translate, 
(DeepL, Amazon) with 
\bs{the widely popular GPT-4 model}
%a widely popular LLM (GPT-4)
in the compelling task of gender-neutral translation, in which avoiding undue (binary) assumptions becomes crucial to promote greater inclusivity in 
%machine-translated texts.
automatically translated texts.
Through extensive fine-grained manual analyses, our study empirically reveals the inherent limitations of current MT systems in generating neutral translations and provides valuable insights into the potential and \ap{the} challenges associated with effectively instructing LLMs for this task.}


==> backup.tex/intro-v1.tex <==

To foster greater inclusivity in our communication practices, there has been a notable rise in the adoption of gender-neutral language strategies across various domains, including institutions \citep{hoglund2023gendering, Euguideline}, academia \citep{apa2020publication}, and industry \citep{microsoft}. These fairer language practices challenge binary gender norms and embrace all gender identities by eschewing gendered terms when they are unnecessary (e.g., \textit{chair} vs chairman/woman). Within the Natural Language Processing (NLP) field, recent advancements have seen the modeling
%integration
of such gender-neutral language principles into monolingual applications \citep{cao2020toward,brandl_how_2022, wagner-zarriess-2022-gender, vanmassenhove-etal-2021-neutral, sun-etal-2019}, also to counter 
%mitigate 
bias and the perpetuation of stereotypes in generative tasks \citep{amrhein2023exploiting}.

Comparatively, however, research has been
scarce for cross-lingual applications, such as the
widely popular Machine Traslation systems (MT).
Existing research in MT has primarily concentrated on gender bias from a strictly binary perspective \citep{savoldi2021gender, lardelli2023genderfair}. As previously argued by \citet{piergentili-etal-2023-gender} and \citep{saunders-byrne-2020-addressing}, however, MT systems often encounter ambiguous input sentences that do not convey any gender distinction (e.g., en:  \textit{I talked to the \textbf{doctors}}). In such cases, the use of neutral and inclusive language becomes imperative to prevent undue (binary) gender inferences in the target language.
So far, 
%Despite these challenges, 
only few individual studies have delved into the topic \citep{cho-etal-2019measuring,piergentili2023hi}, indicating that existing MT systems are ill-equipped for gender-neutral translation. Notably, \citet{saunders-etal-2020-neural} made an attempt to develop inclusive MT models fine-tuned on parallel neutral data for English-Spanish and English-German translation. However, their fine-tuning approach yielded limited success as the models struggled to generalize from a small synthetic adaptation dataset.

The limitations of current MT, coupled with the scarcity of dedicated gender-neutral parallel data to enable supervised approaches for neutral MT, hinder progress in developing more inclusive MT solutions and the broader adoption of MT in contexts that demand gender neutrality. 
Within this landscape, the current LLM paradigm allows to overcome such challenges, by eliciting these models adaptability to perform new (sub) tasks based on explicit instructions and/or a minimal amount of examples. In fact, albeit such language models still lag slightly behind traditional MT systems in terms of overall translation quality \citep{robinson_chatgpt_2023,vilar_prompting_2023,zhang_prompting_2023}, their effectiveness 
%for controlling or 
conditioning specific
%attributes 
%and 
linguistic aspects 
in the output translation has been proven for several attributes \citep{sarti-etal-2023-inseq, moslem_adaptive_2023, garcia_using_2022, yamada_optimizing_2023}, including binary gender forms \citep{sanchez_gender-specific_2023}.
% controlling e.g., formality \citep{Sarti_2023}, terminology \citep{moslem_adaptive_2023}, language variety \citep{garcia_using_2022}, target audience \citep{yamada_optimizing_2023}, and gender, but only binary gender \citep{sanchez_gender-specific_2023}.

In light of the above, this paper aims to advance the automatic generation of gender-neutral translations by exploring feasible approaches to address this task. Specifically, we systematically assess the capabilities of standard MT systems and compare them with those of GPT-4 in generating neutral language for English-Italian translation -— a language pair that presents representative challenges for neutral MT (see section..). Through a series of experiments involving different prompts and shot configurations, whose effectivness is measured by means of extensive, fine-grained analysis, our study shows that \bs{\textbf{aggiustare i findings in base a cosa troviamo, note intanto}}:

\begin{enumerate}
    \item Current MT systems, as well as GPT-4 in zero-shot settings, struggle to perform gender-neutral translation. as corroborated by the study by \citet{ghosh2023chatgpt, savoldi-etal-2022-morphosyntactic, piergentili2023gender}.
    
    \item Prompting GPT-4 yields promising results, with [xxx] achieving the best results
    
    \item The use of in-domain and out-of-domain words selected in the few-shots examples yields varying results, in line with existing literature, which underscores the importance of providing domain-specific examples to enhance task performance...
    
    \item Assessing the acceptability of neutral translations is a highly subjective task, even among evaluators with similar backgrounds and levels of exposure to neutral language. It prompts consideration of procedures for handling annotations with higher subjectivity.
\end{enumerate}

Overall, our study offers valuable insights into the potential and challenges associated with prompting LLMs in the context of gender-neutral translation and lays the groundwork for automating neutral MT. To facilitate future research in this area, we release all manual annotations and judgments of the generated neutral outputs.

==> backup.tex/old-structure.tex <==
\section{Experimental setting}
\label{sec:exp_setting}

%\bs{- QUALI LLM usiamo e perche'}
%\bs{- descrizione dei prompt e motivazione per averli fatti cosi'}
%\bs{- descrizione della valutazione manuale}

%GNT implicates \textit{(i)} understanding whether terms referred to human entities should be gendered and how, and \textit{(ii)} translating them as gender-neutral if that is the case \citep{piergentili-etal-2023-gender}. In our experiments we focus on the second part of the task, to assess whether LLMs are able to produce gender-neutral Italian outputs given neutral English source sentences.

\df{This section describes the data, the models, the prompts, and the evaluation methodology used in our experiments.}

%\subsection{Test data}
%\label{sec:data}
%\hl{[Descrizione di GeNTE]}

\paragraph{Test data.}
%\noindent \textbf{Test data.} 
\bs{discuterei qui le sfide della traduzione per la lingua italian -- se servono -- perche' altrimenti non ci stanno tutti i punti nell'intro}

\ap{\hl{[Zero-shot translation]} For zero-shot translation, we use a subset of Europarl's test set. \textbf{@BEA mandami info su come hai estratto quella porzione please.}}



\ap{For GNT, we use GeNTE \citep{piergentili2023hi}, an en-it parallel corpus designed to evaluate MT models' ability to perform gender-neutral translations. Specifically, we use GeNTE's Set-N, a portion of the corpus which features gender-ambiguous terms in the source sentences that require to be neutrally rendered in translation.}
%There are no informative gender cues associated with human referents in the English source sentences. Therefore we expect each term related human entities to be translated as gender-neutral.

%\bs{Notes: GeNTE is the first test set designed to evaluate MT models' ability to perform gender-neutral translations, but only under desirable circumstances... The corpus consists of 1,500 English-Italian parallel sentences with mentions to human referents, 750 of each (\texttt{Set-N}), feature gender-ambiguous source sentences that require to be neutrally rendered in translation.}

%\subsection{Models}
%\label{sec:models}
%
%\bs{\textbf{Bozza: da aggiustare una ottenuti tutti i risultati finali e in light of stuttura finale del paper.}}
%\smallskip

\paragraph{Models.}
%\noindent \textbf{Models.} 
\df{We test 
three different systems: two commercial systems, Amazon Translate and DeepL, both recognized as leaders in the commercial translation domain, and the latest OpenAI proprietary large multimodal model, GPT-4 \citep{openai2023gpt4}, 
which has demonstrated promising results in translation tasks \citep{jiao2023chatgpt}, though especially for high-resource languages \citep{robinson_chatgpt_2023,stap-araabi-2023-chatgpt}.
GPT-4 belongs to the category of \textit{instruction-tuned} models \citep{chung2022scaling,ouyang_training_2022}, 
which excel in maintaining precise control and adhering to provided guidance, a valuable trait for our gender-neutral translation task.
We prompt these models via their official API. 
In the case of GPT-4, we use the default search strategy with temperature set to $0.0$, since \citet{peng2023making} attested a degradation with high temperature values.}

\bs{PRELIMINARY INFO: in table \ref{tab:translation_quality}, we confirm that GPT however lags behind encoder-decoder MT.}

\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{l|cccc}
 \toprule
 &
  \multicolumn{1}{c}{\textbf{BLEU}} &
  \multicolumn{1}{c}{\textbf{CHRF}} &
  \multicolumn{1}{c}{\textbf{BLEURT}} &
  \multicolumn{1}{c}{\textbf{COMET}} \\
  \toprule
\textbf{Helsinki} &
  \textbf{32.65} &
  \textbf{58.62} &
  \textbf{87.78} &
  \textbf{83.92} \\
  \midrule
\textbf{Amazon}     & 31.04 & 57.54 & 82.84 & 84.07 \\
\textbf{DeepL}      & 30.75 & 56.30 & 82.80 & 83.90 \\
%\textbf{GPT\_bea0}  & 25.40 & 52.04 & 80.83 & 82.92 \\
\textbf{GPT-4} & 25.08 & 51.94 & 80.56 & 82.60 \\
\bottomrule
\end{tabular}
\caption{\bs{Overall quality results. We provide the Helsinki en-it model as an upper-bound.}}
\label{tab:translation_quality}
\end{table}

\paragraph{Prompts.}
%\noindent \textbf{Prompts.} 
\df{\textbf{BOZZA}: For the zero-shot translation task, we adopt \textit{i)} the best resulting prompt by \citep{peng2023making}: \texttt{"Please provide the [TGT] translation of the following sentence:"}.}
%, and \textit{ii)} the more concise \texttt{"Translate into Italian:"}}

\ap{For GNT, we tested three prompts with two sets of shots. Examples of each prompt are available in Table \ref{tab:prompts-in-domain}.}


\ap{• \texttt{contr}: following \citet{sanchez_gender-specific_2023}, we ask the models to provide a contrastive pair of translations for each source sentence -- a gendered one, and a neutral one -- without providing any information about the task.} %The models are supposed to identify the pattern in the examples and to reproduce it.


\ap{• \texttt{CoT-1}: a Chain-of-Thought (CoT) prompt \citep{wei_chain--thought_2023} based on the GNT task description. The system is expected to identify English terms in the source sentence which could possibly be translated as marked in Italian and to elaborate gender-neutral translations before the generation of the final translation.}

\ap{• \texttt{CoT-2}: this CoT replicates how humans instinctively perform GNTs \citep{piergentili-etal-2023-gender,paolucci-etal-2023-gender}, i.e. by first producing a gendered translation and subsequently \textit{neutralizing} gendered terms to produce the final translation.}


\ap{As English emerged as the most effective language for prompting \citep{shi_language_2022,zhang_prompting_2023}, we use English instructions in our prompts, except for the Italian examples in the task demonstrations.} \ap{As for the examples, we developed two sets of shots that differ only for the English terms which require a GNT and their translations into Italian. One set includes terms which exist in the test set, while the other features terms which do not. This allows to investigate the impact of example choice on a complex task of text generation. }
%i.e. whether choosing examples too similar to the test data can lead to overfitting-like scenario.

\begin{table*}[ht]
\scriptsize{
\begin{tabularx}{\textwidth}{lX}
\textbf{Prompt} & \textbf{Example}  \\ \toprule
\texttt{contr} & \begin{tabular}[c]{@{}p{14.5cm}@{}} {[English]}: Several fishermen have joined with the politicians in Belgrade.\\
{[Italian, gendered]}: \textit{\color{blue}A Belgrado, molti pescatori si sono schierati dalla parte dei politici.}\\
\textit{\color{blue}{[Italian, neutral]}: A Belgrado, molte persone che lavorano nella pesca hanno preso le parti di chi fa politica.}\end{tabular} \\ \midrule

\texttt{CoT-1} & \begin{tabular}[c]{@{}p{14.5cm}@{}}Q: Translate the following English sentence into Italian using a gender-neutral language to refer to human entities: [President, everyone must continue to adopt an ambitious approach on these issues.].
\\ A: \textit{\color{blue}In the English sentence [President, everyone must continue to adopt an ambitious approach on these issues.] there are two expressions which refer to human entities and could be translated in a non-neutral way: <President>, and <everyone>. A gender-neutral Italian translation of <President> is <Presidente>. A gender-neutral Italian translation of <everyone> is <ogni persona>. The final gender-neutral translation is [Presidente, su tali questioni sarà necessario che ogni persona continui a dare prova d'ambizione.]}\end{tabular} \\ \midrule

\texttt{CoT-2} & \begin{tabular}[c]{@{}p{14.5cm}@{}}Translate the following English sentence into Italian using a gender-neutral language to refer to human entities: [Secondly, how far does it increase transparency and accountability of the MEPs?]. Think step by step.\\ A: \textit{\color{blue}The English sentence [Secondly, how far does it increase transparency and accountability of the MEPs?] can be translated as [Secondariamente, fino a che punto aumenta la trasparenza e la responsabilità dei parlamentari europei?]. There is one «expression with <non-neutral terms>» that refers to human entities: «<dei parlamentari europei>». A gender-neutral alternative to «<dei parlamentari europei>» is «dei membri del Parlamento Europeo». The final gender-neutral translation is [Secondariamente, fino a che punto aumenta la trasparenza e la responsabilità dei membri del Parlamento Europeo?].}\end{tabular} \\

\end{tabularx}
\caption{\ap{Tentativo di tabella con esempi prompt da inserire nel testo. }Examples for each of the three prompts with in-domain shots. Italicized, blue text indicates the expected output. }
\label{tab:prompts-in-domain}
}
\end{table*}

%\noindent \textbf{Evaluation.}
\paragraph{Evaluation.}

\ap{For general translation quality, we rely on four widely used metrics: BLEU \citep{papineni-etal-2002-bleu}, chrF \citep{popovic-2015-chrf}, BLEURT \citep{sellam-etal-2020-bleurt}, and COMET \citep{rei-etal-2020-comet}.}

\ap{While the GeNTE corpus comes with an associated automatic protocol for GNT evaluation based on a classifier \citep{piergentili2023hi}, we perform a manual analysis of the outputs to overcome two inherent limitations of the classifier. First, it classifies the neutrality of the sentence as a whole, whereas we want to account for each potential neutralization in the sentence. Second, the classifier provides no information on the correctness of the translation and the acceptability of the neutralization. As we are interested in these two crucial aspects, we task three annotators to evaluate them manually.} %\ap{––ANDREA: Secondo me l'esempio qui non è necessario.--}
\ap{The annotators are native Italian speakers with advanced knowledge of gender-neutrality in language and translation. To evaluate gender-neutrality they distinguish among completely neutral, partially neutral, and completely gendered translations. \textbf{Immagino che non riporteremo anche MASC, FEM, MIXED. In caso contrario, correggo.} As for acceptability, the annotators assess whether the neutralizations are both adequate and fluent on a set of four tags which span from unacceptable to acceptable with two degrees of uncertainty in between. \textbf{<-- chiaramente da rivedere anche in base a come riportiamo i risultati.} The evaluation is restricted to the final gender-neutral translation, the rest of the output (e.g., the intermediate steps in the CoTs) is filtered out in postprecessing.}

\ap{\textbf{We compute the IAA...}}
\ap{\hl{Table X} reports the results of the manual evaluation.}

%\bs{TO REMEMBER: We rely on %an automatic 
%\ap{a manual} analysis to overcome 2 inherent limits of the classifier. First, (less important but could be mentioned), it classifies the whole sentence, whereas we want to account for each potential neutralization -- there can be multiple in one sentence. More importantly, however, we do not only want to know if an output translation is NEUTRAL, but if it is a correct/acceptable neutralization. E.g., \textit{I am happy} translated as \textit{sono triste} is neutral, but it is an incorrect translation. Our analysis accounts for this. }



==> backup.tex/prompt-revised.tex <==
To elicit GPT-4 potential for neutral translations, in the 
\textsc{GNT prompting} condition we experiment with three few-shots templates inspired by existing literature on prompting \citep{dong_survey_2023}. As we show in Table \ref{tab:prompts-in-domain}, such prompts are:

%To explore GPT-4 potential for neutral translations in the \textsc{GNT PROMPTING} condition, we experiment with three few-shots prompt templates inspired from existing literature \citep{dong_survey_2023}, which are shown in table \ref{tab:prompts-in-domain}.  

%• 
\textbf{(1)} \textbf{\texttt{Contr}}:  consisting of \textit{contrastive} examples of gendered and neutral translations for each English sentence, without %any 
additional verbalized instructions. Such simple template has shown promising results for controlling the generation of (binary) gender forms with LLaMA \citep{sanchez_gender-specific_2023}. \\
%• 
\indent \textbf{(2)} \textbf{\texttt{CoT-src}}: 
%where \textit{chain-of-thought} demonstrations break the complex tasks into intermediate reasoning that lead to the final output \citep{wei_chain--thought_2023}. In our GNT adaptation, this prompt first guides the identification of \textit{source} terms that correspond to a gendered expression in Italian, and then elaborate on the neutralization of each term to provide the final target translation. \\ 
where \textit{chain-of-thought} demonstrations break complex tasks into intermediate reasoning steps  \citep{wei_chain--thought_2023}. This GNT 
%this 
prompt first guides the identification of \textit{source} terms that correspond to a gendered expression in Italian, then elaborate on the neutralization of each term to provide the final target translation. \\
%
%a Chain-of-Thought (CoT) prompt \citep{wei_chain--thought_2023} based on the GNT task description. The system is expected to identify English terms in the source sentence which could possibly be translated as marked in Italian and to elaborate gender-neutral translations before the generation of the final translation.
%
%
\indent \textbf{(3)} \textbf{\texttt{CoT-tgt}}: 
unlike \texttt{CoT-src}, this template emulates
% unlike \texttt{CoT-src}, this template emulates 
how humans approach neutralization for monolingual post-editing scenarios \citep{paolucci-etal-2023-gender}, i.e. 
Namely, 
by identifying in 
%\df{identifies in }
an intermediate gendered translation which \textit{target} terms are to be neutralized in the final translation. 

Each of this prompt is used with 3-shots exemplars and sentences taken from the institutional domain,
%Such is in fact the domain represented in GeNTE, and in which neutral language is typically employed \citep{piergentili2023hi}. 
the context where neutral language is conventionally employed and is also utilized in GeNTE.
%Howeber, to
To 
verify GPT-4's ability to generalize from the provided examples, we experiment with two sets of sentences, which only differ for the inclusion of terms to be neutralized that 
\textit{i)} are included and \textit{ii)} never occur in GeNTE (see Appendix \ref{app:prompts}).
%\textit{i)} are included in GeNTE, and \textit{ii)} terms that never occur in the test set (see Appendix \ref{app:prompts} for detailed information.)




==> limitations-bea.tex <==
- prospettiva soggetivita'
You11:50 AM
==> per il futuro contare se agr = o maggiore su automatic neutral translations vs human translations

===================================================================================
In the paper, we have conducted a first investigation to advance the task of gender-neutral translation by verifying a first potential solution towards enabling automatic GNT. To do so, we had to restrict our focus and experiments on what was deemed as necessary for a first step in such a direction, and left several considerations for future work. Naturally, this comes with several limitations. 


\paragraph{One language pair.} Our experiments are carried out for the English$\rightarrow$, and we are thus cautious to indiscriminately generalize our findings. 
%our findings to languages with different typological features and sociolinguistic considerations towards inclusive language. 
Nonetheless, Italian was chosen as a highly representative example of the challenges faced in cross-lingual transfer from English. Accordingly, we believe that our observations (e.g., ascertained GNT capabilites of GPT-4, the subjective evaluation of GNT) can broadly apply to other target grammatical gender languages for high-resource scenarios, too. 
Crucially, the decision to work on English$\rightarrow$ was determined by the fact that -- to the best of our knowledge -- the bilingual GeNTE corpus \S(\ref{sec:exp_setting}) is the only available resource for testing GNT in naturalistic conditions and on several phenomena. The only other resource being the sythentic dataset by \citet{cho-etal-2019measuring}, which however only focuses on preserving \textit{pronouns} neutrality for English$\rightarrow$Korean. 

\paragraph{Closed-source models.} The study relies on different closed-source models: Amazon Translate, DeepL and GPT (\texttt{gpt-4-0613}). This has reproducibility consequences, since these models are regularly updated, thus potentially yielding future  results that differ from those reported in this paper. Also, their access via API (paid in US dollars) might not be affordable for all institutions/researchers.  As a first attempt to a new, complex task with relevant societal impatc such as GNT, we considered reasonable to \textit{i)} focus on general-purpose models used as scale by milions of users, and to which we had access; \textit{ii)} experiment GNT prompting on the strong GPT model, which as of October 2023 holds the first position on the AlpacaEval leaderboard.\footnote{An Automatic Evaluator for Instruction-following Language Models: \url{https://tatsu-lab.github.io/alpaca_eval/}.}
In future work, we plan to test and compare open-source models for this task.\footnote{We conducted experiments with the instruction-following, encoder-decoder bases \texttt{Flan-T5 XXL model}\citep{longpre2023flan}\footnote{\url{https://huggingface.co/google/flan-t5-xxl}.}. Its low translation quality for en-it, however, did not make it a suitable candidate for GNT.}, and  investigate  how to weight the strengths of traditional, dedicated MT systems (i.e. higher translation quality) with those of LLMs (i.e. adaptability to neutral constrains).

\paragraph{Prompts configurations and settings.} 
The three prompts designed in the study are drawn from well-attested, efficient prompt from the literature, which make for reasonable comparisons. While we note that the most successful GNT prompts (\texttt{contr} and \texttt{cot-tgt}, see \S\ref{sec:gnt-results}) imply the inclusion of a contrastive/intermediate gendered translation, we do not necessarily advocate for future approaches to GNT as a monolingual, rewriting step applied to the gendered translation only. Rather, by design, in this work we only experimented with gender-ambiguous source sentences (e.g., \textit{all doctors}), which all require to be neutralize in the target language. However, in line with \citep{piergentili-etal-2023-hi}, we regard GNT as not necessarily desirable under all circumstances, such when the gender of the referents is known and expressed (e.g., \textit{\textbf{She}} \textit{is a doctor}). To make such a distinction, it is pivotal to consider the source English sentence, and we plan to incorporate such scenarios in future experimental settings. Also, we tested the use of in-domain and out-of-domain gender terms in the prompt examples sentences (\S\ref{sec:gnt-prompting}), so to investigate GPT's ability to generalize from the given examples. We recognize that a more comprehensive investigation of GPT's generalization ability woul advocate for the use of example sentences e.g. from varying domains, with more radical structural and stylistic differences. However, for this first exploration we followed 
%As our study is a first exploration of GNT prompting, we relied on 
existing literature on prompt engineering for MT, which advocates for the choice of demonstrations based on the stylistic and semantic similarity \citep{zhang_prompting_2023,vilar_prompting_2023,agrawal_-context_2023}.
%We leave the exploration of different approaches to task demonstrations to future work.

% Also, we experiment   

% In our study we used in-domain and out-of-domain sets of examples. However they only differ for the use of specific terms, whereas the rest of the sentence is identical. A more comprehensive investigation of GPT's ability to generalize would require the use of completely different sentences in both syntax and semantics. As our study is a first exploration of GNT prompting, we relied on existing literature on prompt engineering for MT, which advocates for the choice of demonstrations based on the stylistic and semantic similarity with the output \citep{zhang_prompting_2023,vilar_prompting_2023,agrawal_-context_2023}. We leave the exploration of different approaches to task demonstrations to future work.

\paragraph{The subjectivity of the GNT task.}




bs{why not usare LLMs per valutazione}
\ap{Using LLMs for the automatic evaluation of natural language generation is possible and productive \citep{liu_g-eval_2023,wang2023chatgpt,fu2023gptscore}. However, the evaluation of a complex task such as GNT is still unexplored. It requires an empirical investigation of prompting strategies, similar to the one presented in this work. Before venturing into the exploration of this possibility we found it more appropriate and significant to first assess whether LLMs were able to perform the task, rather than evaluate it. LLM-based evaluation pipelines represent a promising future direction for GNT evaluation, we will explore it in future work. \textbf{È un po' una lunga supercazzola ma la rivediamo.}} 

% \bs{dominio/non dominio} \ap{In our study we used in-domain and out-of-domain sets of examples. However they only differ for the use of specific terms, whereas the rest of the sentence is identical. A more comprehensive investigation of GPT's ability to generalize would require the use of completely different sentences in both syntax and semantics. As our study is a first exploration of GNT prompting, we relied on existing literature on prompt engineering for MT, which advocates for the choice of demonstrations based on the stylistic and semantic similarity with the output \citep{zhang_prompting_2023,vilar_prompting_2023,agrawal_-context_2023}. We leave the exploration of different approaches to task demonstrations to future work.}


%\bs{Only one language} \ap{Our study is limited to only one language pair. This is due to the lack of resources dedicated to GNT in other language pairs. The en-it pair is however representative of a crucial scenario for GNT, i.e. where the target language is characterized by an extensive grammatical gender system.}

% \ap{Finally, for our experiments we only tested one commercial, decoder-only, closed-source LLM: GPT-4. As a first attempt at a new task with an experimental approach we deemed reasonable to turn to the model which performs best in many NLG tasks: as of September 25th 2023, GPT-4 holds the first position on the AlpacaEval leaderboard.\footnote{An Automatic Evaluator for Instruction-following Language Models: \url{https://tatsu-lab.github.io/alpaca_eval/}.} We plan to test and compare other models in the future, including open-source and encoder-decoder LLMs and MT systems.}


In Table \ref{}, we report the scores measured with the official GenTE automatic evaluation protocol by all models and GPT configurations used in our main experiments.

As such accuracy scores stand  contrast with the results of our manual analysis (e.g., consistent number of generated GNTs for the MT systems), we decided to further verify the reliability of such an evaluation by \textit{i)} calculating percentage agreement against the ground truth label on gender-neutrality obtained via our manual evaluations (see Table \ref{tab:classifier}, and \textit{ii)} computing Kendall's 
correlation coefficient ($\tau$) on the rankings resulting from the classifier and manual analysis. \footnote{Calculated with SciPy; \url{https://scipy.org/}} 

